Beyond the Code: Mining Self-Admitted Technical Debt in Issue Tracker Systems

Self-admitted technical debt (SATD) is a particular case of Technical Debt (TD) where developers explicitly acknowledge their sub-optimal implementation decisions. Previous studies mine SATD by searching for specific TD-related terms in source code comments. By contrast, in this paper we argue that developers can admit technical debt by other means, e.g., by creating issues in tracking systems and labelling them as referring to TD. We refer to this type of SATD as issue-based SATD or just SATD-I. We study a sample of 286 SATD-I instances collected from five open source projects, including Microsoft Visual Studio and GitLab Community Edition. We show that only 29% of the studied SATD-I instances can be tracked to source code comments. We also show that SATD-I issues take more time to be closed, compared to other issues, although they are not more complex in terms of code churn. Besides, in 45% of the studied issues TD was introduced to ship earlier, and in almost 60% it refers to Design flaws. Finally, we report that most developers pay SATD-I to reduce its costs or interests (66%). Our findings suggest that there is space for designing novel tools to support technical debt management, particularly tools that encourage developers to create and label issues containing TD concerns.

==> tex/related-work-backup.tex <==
\section{Related Work}
\label{sec:related-work}
%General
Rios~\textit{et al.}~\cite{rw21} conduct a tertiary study on technical debt and investigates the current state of research on TD. Sierra~\textit{et al.}~\cite{rw16} also conduct a literature survey, although they concentrated on self-admitted technical debt (SATD) and analyses various empirical studies that have focused on investigating source code comments that indicate SATD. However, to the best of our knowledge, we are the first to study self-admitted technical debt (SATD) in issues.  

There are several studies in the literature that the central purpose is the identification of technical debts. Flisar and Podgorelec~\cite{rw11}, Huang~\textit{et al.}~\cite{rw12}, Ren~\textit{et al.}~\cite{rw13}, and Fahid~\textit{et al.}~\cite{rw17} use machine learning techniques for automating the detection of SATD. Huang~\textit{et al.}~\cite{rw12} and Liu~\textit{et al.}~\cite{rw14} identify SATD from source code comments using text mining, and Dai and Kruchten~\textit{et al.}~\cite{rw15} also adopt machine learning techniques and  natural language processing for identifying technical debts, but their approach finds identifying non-code-level technical debt through issue tracking data sets.

Other studies explore the impacts of technical debts on the software development lifecycle. Becker~\textit{et al.}~\cite{rw18}\cite{rw19} investigate the consequences of TD in terms of wastage of development time, Martini~\textit{et al.}~\cite{rw22} investigates the state of practice in several companies to understand what the cost of managing TD is, what tools they use to track TD, and how to introduce a tracking process in practice, and Maldonado~\textit{et al.}~\cite{rw20} investigate for how long SATD lives in a project and what activities lead to the removal of SATD.

%1 - Is Self-Admitted Technical Debt a Good Indicator of Architectural Divergences?
Sierra~\textit{et al.}~\cite{rw1} investigates the possibility of using source code comments that indicate Technical Debt, i.e., Self-Admitted Technical Debt (SATD), to resolve architectural divergences. The authors used a data set of previously classified SATD comments to trace them to the architectural divergences in {ArgoUML}, an open-source system. They found 7 high-level divergences in {ArgoUML} and 22 others among its subsystems, observing that only 4 out of 29 (14\%) divergences can be directly traced to SATD comments. For the authors, it is viable to use SATD comments as an indicator of architectural divergences, however, the effort is high, and in general, will not lend to a significant reduction of architectural flaws in a software system.

% 3 Using Natural Language Processing to Automatically Detect Self-Admitted Technical Debt
Maldonado~\textit{et al.}~\cite{rw3} proposes an approach to automatically identify design and requirement SATD using Natural Language Processing (NLP). Using 10 open source projects, they were able to precisely identify SATD and significantly outperforming the current state-of-the-art based on fixed keywords and phrases. They achieved 90\% of the best classification performance, using only 23\% of the comments for both design and requirement SATD, and 80\% of the best performance, using only 9\% and 5\% of the comments for design and requirement SATD, respectively. These findings show that their approach can achieve good accuracy even with a small training dataset.

% 4 The Pricey Bill of Technical Debt - When and by whom will it be paid?

Besker~\textit{et al.}~\cite{rw4} estimate wasted time caused by the Technical Debt interest during the software life-cycle, and investigate how practitioners perceive and estimate the impact of the negative consequences due to Technical Debt during the software development process. Their findings show that, on average, developers waste 36\% of all development time due to Technical Debt, and most this time is wasted on understanding the Technical Debt. The authors also observed that the consequences of Technical Debt are also influenced by the age of the software system, and Complex Architectural Design and Requirement Technical Debt generates the most negative effects.

% 5 A Large-Scale Empirical Study on Self-Admitted Technical Debt
Bavota and Russo~\cite{rw5} investigates the diffusion and evolution of SATD and its relationship with software quality. The authors mined over 600K commits and 2 Billion comments and performed a qualitative analysis via open coding. Their main finding shows that SATD is diffused, with an average of 51 instances per system, where the most diffused type of SATD is code debt (30\% of instance), followed by defect and requirement debt (20\% each) and design debt (13\%).  The authors also observe that SATD increases over time due to the introduction of new instances that are not fixed by developers, and even when fixed, it survives a long time (over 1,000 commits on average) in the system.

% 6 - An Exploratory Study on Self-Admitted Technical Debt
Potdar and Shihab~\cite{potdar2014} analyzed four large open-source projects. The study assess self-admitted technical debt and the main reasons related to their creation. The results reported that 2.4\% - 31\% of source code files contain self-admitted technical debt and experienced developers tend to introduce more debts. Lastly, the authors also identified the only  26.3\% - 63.5\% of addresses self-admitted debt gets removed by maintainers after the introduction.

%7 - Exploring the costs of technical debt management – a case study
In another study, Guo~\textit{et al.}~\cite{rw7} focused on the cost of managing technical debts, the study proposes a new method for managing technical debts.  The authors evaluated the approach in a study case in a real software project. Reported results show that the technique increases 70\% of the sprint planning effort in the first release cycle. However, the approach provides good insights for project management and supports organizations in decisions making in future projects.

% 8 - Examining the Impact of Self-admitted Technical Debt on Software Quality
Sultan~\textit{et al.}~\cite{rw8} assess the impact of self-admitted technical debt on software quality. In an empirical study, the authors analyzed five popular open-source projects. The key findings show no relation between technical debt and defects. However, the results reveal negative effects in software maintenance, making systems more difficult to change in the future.

% 9 - Detecting and Quantifying Different Types of Self-Admitted Technical Debt
In a recent study, Maldonado and Shihab~\cite{rw9} examined 33K code comments from five open-source projects. The study classified self-admitted technical debt into five categories:  design debt, defect debt, documentation debt, requirement debt, and test debt. The most common type recorded is design debt, which is present in 42\% to 84\% of analyzed comments followed by requirement debt, 5\% to 45\% of comments.

% 10. Measure It? Manage It? Ignore It? Software Practitioners and Technical Debt 
Ernst~\textit{et al.}~\cite{rw10} reported a survey and a follow-up interview with 1831 experienced software engineers and managers from three large organizations. The study indicates that architectural decisions are one of the most important sources of technical debt. Furthermore, results show a fault of tools to manage technical debt and standard practices to support professionals.




